Generative Entity Typing with Curriculum Learning

Entity typing aims to assign types to the entity mentions in given texts. The traditional classification-based entity typing paradigm has two unignorable drawbacks: 1) it fails to assign an entity to the types beyond the predefined type set, and 2) it can hardly handle few-shot and zero-shot situations where many long-tail types only have few or even no training instances. To overcome these drawbacks, we propose a novel generative entity typing (GET) paradigm: given a text with an entity mention, the multiple types for the role that the entity plays in the text are generated with a pre-trained language model (PLM). However, PLMs tend to generate coarse-grained types after fine-tuning upon the entity typing dataset. Besides, we only have heterogeneous training data consisting of a small portion of human-annotated data and a large portion of auto-generated but low-quality data. To tackle these problems, we employ curriculum learning (CL) to train our GET model upon the heterogeneous data, where the curriculum could be self-adjusted with the self-paced learning according to its comprehension of the type granularity and data heterogeneity. Our extensive experiments upon the datasets of different languages and downstream tasks justify the superiority of our GET model over the state-of-the-art entity typing models. The code has been released on https://github.com/siyuyuan/GET.

==> 030Preliminary.tex <==
\section{Preliminaries}\label{sec:Preliminaries}
We formalize our task in this paper and then present how to collect the training data in this section.
\subsection{Task Definition}
Given a piece of text $X$ and an entity mention $M$ within it, the task of {\bf generative entity typing (GET)} is to generate multiple types $TS=\{T_1, T_2, ..., T_K\}$, where each $T_k (1\leq k\leq K)$ is a type for $M$ w.r.t. the context of $X$. 

\subsection{Data Collection}\label{sec:data}
To train a desirable PLM-based GET model, we need adequate training data with high-quality and fine-grained types as many as possible.
However, due to the difficulty and high cost of human annotation, most existing works generally adopt heterogeneous data consisting of a small portion (less than 10\%) of human-annotated data and a large portion (more than 90\%) of \dqyang{low-quality data automatically generated by} distant supervision~\cite{gong2021abusive}. 

In this paper, we also adopt heterogeneous data in which the human-annotated data \dqyang{was directly} collected from the existing work~\cite{choi2018ultra,lee2020chinese}, and a large number of high-quality auto-annotated samples were obtained from the abstracts of entities on Wikipedia~\cite{vrandevcic2014wikidata}. 
Specifically, we collected the abstract texts and their hyperlinks pointing to the mentioned entities' web pages, from which the type labels of these mentioned entities could be obtained.
In this way, the obtained type labels are more consistent with the entities' contexts, and thus of much higher quality than those auto-generated with distant supervision~\cite{gong2021abusive}.

